Quantum phases of hardcore bosons in two coupled chains: A density matrix renormalization group study

We consider hardcore bosons in two coupled chain of one dimensional lattices at half filling with repulsive intra-chain interaction and inter-chain attraction. This can be mapped on to a coupled chain of spin-1/2 XXZ model with inter chain ferromagnetic coupling. We investigate various phases of hardcore bosons (and related spin model) at zero temperature by density matrix renormalization group method. Apart from the usual superfluid and density wave phases, pairing of inter chain bosons leads to the formation of novel phases like pair-superfluid and density wave of strongly bound pairs. We discuss the possible experimental realization of such correlated phases in the context of cold dipolar gas.

==> report.tex <==
To
Dr. Robert Konik
Associate Editor
Physical Review B

         Dear Dr.Robert Konik

                      Thank you very much for your email, with reviewers comments on our manuscript entitled 
" Quantum phases of hardcore bosons in two coupled chains: A DMRG study", authored by Bradraj Pandey, Subhasis Sinha and Swapan K Pati.
 We have considered all the comments of the two reviewers and have modified our manuscript accordingly. 
We hope our revised manuscript would be suitable for Physical Review B and we hope to hear from you soon.
Thank you very much.
with our best regards.
Swapan K Pati

 In the  revised manuscript, the changes made are written in bold.  Almost in all the pages, we have made changes.

We also have made the follwing changes:
1. We have included some references suggested by the reviewers and have discussed in the text.
2. Axes labels U and V are corrected.
3. An additional Fig describing power law fitting of correlation function in a log-log scale is given (Fig.5c)  
4. Insets of Fig.4 and Fig.8 have been replotted with additional input parameters.

We are uploading the following files:

1. Modified manuscript
2 Reply to each of reviewers in separate files (2 files)

Hope you will find the files in order and the answers will satisfy the reviewers.

Hope to here from you very soon
Thanking you and with our best regards,
Swapan K Pati


